Graph Profiling for Vertex Cover: Targeted Reductions in a Branch and Reduce Solver

Akiba and Iwata [TCS, 2016] demonstrated that a branch and reduce (B&R) solver for the vertex cover problem can compete favorably with integer linear programming solvers (e.g., CPLEX). Our research question is are there graph characteristics that determine which reductions will be most effective? Not only is the answer affirmative, but relevant characteristics are easy to identify. To explore our ideas, we provide an enhanced version of the Akiba-Iwata solver that can (a) be configured with any subset of reductions and lower bounds; (b) print statistics such as time taken and number of vertices reduced by each reduction. Based on extensive experiments with benchmark and random instances we demonstrate that (i) more reductions do not necessarily lead to better runtimes; (ii) the subset of reductions leading to the best (or nearly the best) runtime can be predicted based on measurable characteristics of a graph, e.g., density and degree distribution; and (iii) exceptions have structural characteristics known in advance. Our primary contributions are 1. A thorough examination reduction routine performance in the context of graph characteristics. 2. Three primary hypotheses suggesting simple suites of reductions as the most efficient options. 3. Experiments with a large corpus of data to validate our hypotheses. 4. Measures that quantify a problem instance on two key dimensions to make our hypotheses concrete. 5. An enhanced open-source version of the Akiba-Iwata solver that enables our investigations and creates opportunities for future exploration. Our main objective is to provide guidance to a user so that, faced with a given problem instance or set of instances, they may most effectively use the available reductions. Ultimately these efforts can lead to an automated process.

==> 4-sparse_real_world.tex <==
The large sparse real-world graphs reported in \cite{Akiba} require
additional care.
Because of their size, it is important to reduce as many vertices as possible
early on to avoid massive branching.
The simple reductions won't do the trick but we can take a lesson from the
observed effectiveness in
Table~\ref{tab:reduction_effectiveness_efficiency}(a).
Unconfined reductions are useful on their own and have the additional advantage
that they generalize \domRed{}.
LP reductions are especially effective on larger graphs because they
(a)~reduce many vertices at once; and (b)~are linear time after the
construction of the auxiliary graph and a maximum matching at the root.

So for these graphs we added the \textsf{Cheap+LPU} configuration, which is
\textsf{r2\_l4} without \domRed{} and \funnelRed.
This has the effect of postponing \domRed until after the cheaper ones and
avoiding the pitfalls of \funnelRed reductions -- these can significantly
increase the number of edges while removing only two vertices. For an
egregious example, see Appendix~\ref{app:mann}. 

% [Last modified: 2019 08 11 at 21:23:37 GMT]


==> A-configs.tex <==
\input{Y-configs}

\cmt{add text, some lifted from footnotes}

% [Last modified: 2020 02 18 at 15:27:26 GMT]


==> A-mann.tex <==
\cmt{This is dangling now -- it was supposed to illustrate a case where
  adding a reduction (funnel) can wreak havoc and supports an argument for
  using, e.g., \cheapLPU instead of \rtlf}

The \textsf{MANN} instances, derived from Steiner triples \cmt{citation},
have many vertices of high degree (e.g., vertex~1 in Fig.~\ref{fig:funnel_MANN_a9} -- outlined in red),
each
    adjacent to multiple triangles.
    The only reductions that apply to the original instance are funnel
    reductions. These introduce $K_{2,k-1}$ subgraphs, where $k$ is the
    degree of the high degree vertex.
    For \textsf{MANN\_a}$\beta$, $k=4,13,22,40$ when $\beta=9,27,45,81$,
    respectively.
    
    However, if \funnelRed{} reductions are not applied, when a degree-$k$ vertex
    is removed during branching, its neighbors have degree~2: they and the
    triangles in which they appear are removed by the degree-2 dominance
    reductions enabled during a \foldRed{}.
    In fact, the best runtime is achieved for the \textsf{MANN} instances
    when \foldRed{} only is applied. See Table~\ref{tab:funnel_MANN}.
    The \textsf{r2\_l4} configuration times out on \textsf{MANN\_a45} while
    \foldRed{} finishes in 9~seconds. 

\begin{figure}[h]
  \centering

  \includegraphics[width=\columnwidth]{funnel_MANN_a9-before.png}

  (a)~Closeup of a subgraph of \textsf{MANN\_a9} before \funnelRed.

  \medskip
  
  \includegraphics[width=\columnwidth]{funnel_MANN_a9-after.png}

  (b)~The subgraph from part~(a) after \funnelRed.

  \caption{Effect of a funnel reduction on a \textsf{MANN} instance.}
  \label{fig:funnel_MANN_a9}
\end{figure}

\begin{table}[h]
  \small
  \caption{Adding a (funnel) reduction can significantly increase the number of
    branches.}
  \label{tab:funnel_MANN}

  \medskip
  \centering
  \begin{tabular}{|l||r|r|r|}
    \hline
    \textsf{MANN\_a27} & \foldRed{} & \textsf{r0\_l1} & \textsf{r2\_l4} \\
    \hline
    branches & 6,212 & 5,766 & 10,797 \\
    \hline
    runtime & 0.33 & 0.49 & 4.08 \\
    \hline
  \end{tabular}
\end{table}

% [Last modified: 2020 02 18 at 17:46:41 GMT]


==> Y-blg_exceptions_table.tex <==
\begin{table*}
  \small
  
  \caption{Runtimes for exceptions.}
  \label{tab:blg_exceptions}

  \cmt{Some table entries, especially the min column, are incorrect or
    incorrectly identified (italics should be used for runtimes within a
    factor of 2).}
  
  \begin{center}
    \medskip

    \begin{tabular}{|r|r|r|r|r|r|r|r|r|r|}
      \hline \hline
      \multicolumn{10}{|c|}{Instances where \cheap{} config is competitive in \none{} region.} \\ \hline
      spread & nad & None & Deg1 & DD & Cheap & LP & All & CPLEX & min\\\hline
      0.69 & 160 & \emph{1.25} & \textbf{0.79} & \emph{1.52} & \textbf{1.01} & 1.99 & 2.37 & 15.01 & 0.79\\\hline
      0.70 & 160 & 1.53 & \textbf{1.06} & 1.61 & \textbf{0.81} & 2.22 & 2.24 & 10.21 & 0.81\\\hline
      0.24 & 160 & \emph{1.74} & \emph{1.87} & \textbf{1.36} & \textbf{0.97} & \textbf{1.16} & 2.56 & 60.86 & 0.97\\\hline
      0.01 & 160 & \emph{2.25} & \textbf{1.40} & \emph{2.29} & \textbf{1.23} & \emph{2.25} & 2.94 & 76.96 & 1.23\\\hline
      \\\hline
      \multicolumn{10}{|c|}{Instances where \all{} config is best but in \cheap{} region.} \\ \hline
      spread & nad & None & Deg1 & DD & Cheap & LP & All & CPLEX & min\\\hline
      1.32 & 20 & 8.82 & 9.49 & 5.53 & 10.90 & 14.75 & \textbf{3.36} & 0.07 & 5.53\\\hline
      1.48 & 20 & 6.70 & 6.73 & \emph{3.83} & 8.19 & 11.39 & \textbf{2.41} & 0.07 & 6.70\\\hline
      1.47 & 20 & 7.38 & 7.53 & \emph{4.15} & 9.33 & 13.09 & \textbf{2.02} & 0.06 & 7.38\\\hline
      1.38 & 20 & 8.50 & 9.24 & \emph{4.83} & 11.47 & 16.50 & \textbf{2.93} & 0.10 & 8.50\\\hline
      1.38 & 20 & 10.16 & 10.53 & \emph{4.59} & 11.42 & 17.90 & \textbf{2.82} & 0.07 & 10.16\\\hline
      1.26 & 20 & 11.26 & 13.15 & \textbf{7.78} & 14.42 & 20.71 & \textbf{6.72} & 0.12 & 11.26\\\hline
      1.23 & 20 & 11.65 & 11.96 & \emph{7.39} & 14.26 & 20.87 & \textbf{4.86} & 0.10 & 11.65\\\hline
      1.37 & 20 & 11.83 & 11.83 & \textbf{5.45} & 15.23 & 21.05 & \textbf{4.32} & 0.03 & 11.83\\\hline
      1.17 & 20 & 13.99 & 14.32 & \emph{10.37} & 17.38 & 24.01 & \textbf{6.05} & 0.07 & 13.99\\\hline
    \end{tabular}
  \end{center}
\end{table*}

% [Last modified: 2019 06 25 at 20:34:13 GMT]


==> Y-blg_exclusive.tex <==
\begin{figure*}
  \centering
  \begin{minipage}{\textwidth}
    \begin{tabular}{c @{~~} c}
      \includegraphics[width=0.45\textwidth]{blg-exclusive.pdf}
      &
      \begin{minipage}[b]{0.45\textwidth}
        In this and all future scatterplots like it, the x-axis represents
        degree spread and the y-axis normalized average degree (log scale).
        The intent is to show regions in the landscape defined by these two
        coordinates in which each of the given configurations is the only
        competitive one.
        \cmt{need to draw regions}
      \end{minipage}
    \end{tabular}
  \end{minipage}
  \caption{Scatterplot showing regions where each of three configurations is
    exclusively competitive.}
  \label{fig:blg_exclusive}
\end{figure*}

% [Last modified: 2020 02 18 at 17:47:14 GMT]


==> Y-blg_scatter.tex <==
\begin{figure}
  \centering
  \begin{minipage}{\textwidth}
    \begin{tabular}{c c}
      \includegraphics[width=0.4\textwidth]{blg-centroids.pdf}
      &
      \includegraphics[width=0.7\textwidth]{blg-heatmap.pdf}
      \\
      (a)~competitive reduction sets & (b)~criticality heatmap
    \end{tabular}
  \end{minipage}
  \caption{Scatterplots showing competitive reduction sets for our random instances.}
  \label{fig:blg_scatter}
\end{figure}

% [Last modified: 2020 02 18 at 17:47:33 GMT]


==> Y-branching.tex <==
\begin{table}
  \small
  \caption{Situations where adding reductions increases the number of
    branches.}
  \label{tab:branching}

  \medskip
  \centering
  \begin{tabular}{|l||r|r|r|r|}
    \hline
    \textsf{MANN\_a27} & \textsf{r0\_l1} & \textsf{r1\_l4} & \textsf{r2\_l4} & \textsf{r3\_l4}\\
    \hline
    branches & 5,766 & 5,730 & 10,797 & 2,771\\
    \hline
    runtime & 0.49 & 0.56 & 4.08 & 1.83 \\
    \hline\hline
    \textsf{aa20-to} & \textsf{r0\_l1} & \textsf{r1\_l4} & \textsf{r2\_l4} & \textsf{r3\_l4}\\
    \hline
    branches &  132,628 &  3,036 & 2,979 & 162,581 \\
    \hline
    runtime  & 18.81 &	2.71 &	3.80 & 63.79 \\
    \hline
  \end{tabular}

  \medskip
  \begin{minipage}{\textwidth}
    For the \textsf{MANN\_a27} instance it is clear that adding more reductions
    can significantly increase the number of branches.
    While most reductions have no effect initially with the \textsf{MANN}
    instances \cmt{refer to figure and detailed decription in Appendix?}, removal of the highest degree
    vertices by branching leaves a collection of triangles, which are reduced via
    dominance. Other reductions, however, may reduce the degree of these critical
    branching vertices, leading to smaller instances with less desirable
    structure.
    In this case, the only reductions that take place at the root are funnel
    reductions.

    \textsf{aa20-to} has relatively few odd cycles, making LP reductions
    effective. The packing reduction appears to create problems \cmt{reasons
      not clear.}
  \end{minipage}

\end{table}

% [Last modified: 2019 07 17 at 17:38:36 GMT]


==> Y-cheap-table.tex <==
\begin{table*}
  \caption{Selected instances in the \cheap{} region.}
  \label{tab:cheap-table}
    \begin{tabular}{|r|r||r|r|r|r|r|r|r|r|}
      \hline
      spread & nad & None & Deg1 & DD & Cheap & LP & All & CPLEX & min\\\hline
2.67 & 5 & 85.47 & 2.91 & 3.28 & \textbf{0.22} & 1.03 & 0.52 & 1.16 & 0.23\\\hline
0.00 & 3 & 900.00 & 900.00 & 900.00 & \textbf{0.61} & 5.43 & 1.15 & 1.45 & 0.61\\\hline
0.00 & 3 & 900.00 & 773.92 & 797.86 & \textbf{0.68} & 10.56 & 1.09 & 1.49 & 0.69\\\hline
4.80 & 20 & 15.83 & 3.20 & 3.70 & \textbf{1.36} & 4.24 & 4.35 & 26.40 & 1.37\\\hline
4.88 & 40 & 3.19 & 2.26 & 2.32 & \textbf{1.74} & 2.84 & 6.28 & 18.21 & 1.75\\\hline
7.03 & 40 & 900.00 & 198.03 & 213.17 & \textbf{2.68} & 27.22 & \emph{4.09} & 14.87 & 2.69\\\hline
5.11 & 10 & 857.53 & 214.69 & 226.37 & \textbf{6.94} & 36.51 & 13.67 & 40.77 & 6.94\\\hline
5.99 & 10 & 900.00 & 900.00 & 900.00 & \textbf{18.19} & 199.12 & 29.39 & 28.05 & 18.19\\\hline
7.29 & 10 & 900.00 & 900.00 & 900.00 & \textbf{55.13} & 381.11 & \emph{84.55} & 106.36 & 55.13\\\hline
0.00 & 7 & 325.67 & 230.12 & 242.26 & \textbf{81.02} & 176.86 & \emph{132.55} & 151.33 & 81.02\\\hline
    \end{tabular}
\end{table*}

% [Last modified: 2019 06 25 at 20:20:29 GMT]


==> Y-coding_theory.tex <==
\begin{table}
  \caption{Runtime data for coding theory instances.}
  \label{tab:coding_theory}

  \medskip
  \begin{tabular}{|l||r|r|r|r||r|r|r|r|r|}
    \hline
    Instance & n & m & spread & nad & None & DF2 & r0\_l1 & min & CPLEX \\ \hline
    1et.512 & 510 & 4,032 & 3.4 & 15.8 & 3.39 & 3.26 & 2.95 & 2.89 & 2.33 \\ \hline
    1tc.512 & 510 & 3,264 & 5.5 & 12.8 & 2.60 & 2.01 & 1.09 & 0.88 & 0.17 \\ \hline
    1zc.128 & 128 & 1,120 & 1.5 & 17.5 & 21.77 & 20.89 & 7.52 & 7.52 & 0.10 \\ \hline
    2dc.512 & 512 & 54,895 & 2.7 & 83.8 & 24.02 & 25.29 & 5.62 & 5.62 & 45.22 \\ \hline
  \end{tabular}

  \medskip
  \begin{minipage}{\textwidth}
    In the first three instances, DF2 is expected to be competitive.
    The two cases where it is not, 1tc.512 and 1zc.128 are solved easily at
    the root by CPLEX.
    The last instance, where one would expect not to have to do any
    reductions, has many dominance relationships. \cmt{refer to Yang's
      thesis; I think all of these have dominance relationships by design.}
  \end{minipage}
\end{table}

% [Last modified: 2019 07 25 at 20:10:39 GMT]


==> Y-geo_512_table.tex <==
\begin{table*}
  \caption{Data for geometric graphs with 512 vertices.}
  \label{tab:geo_512}

  \medskip
  \centering
  \small
  \begin{tabular}{|r|r|r||r|r|r|r|r||r|r|r|r|}
    \hline
    edges & spread & nad & DD & r0\_l1 & r0\_l1+U & CPLEX & min & DD & r0\_l1 & r0\_l1+U & CPLEX \\ \hline
    1,201 & 4.0 & 4.7 & 0.01 & 0.01 & 0.01 & 0.06 & 0.01 & 13 & 1 & 1 & 1 \\ \hline
    \hline
    1,964 & 4.3 & 7.7 & 0.03 & 0.01 & 0.01 & 0.07 & 0.01 & 141 & 1 & 1 & 1 \\ \hline
    \hline
    3,747 & 3.1 & 14.6 & 7.84 & 0.81 & 0.07 & 0.14 & 0.07 & 129,551 & 2,367 & 29 & 1 \\ \hline
    \hline
    7,161 & 2.7 & 10.9 & 13.01 & 6.48 & 0.56 & 0.58 & 0.56 & 179,229 & 38,691 & 431 & 10 \\ \hline
    \hline
    13,547 & 2.7 & 20.7 & 0.73 & 0.70 & 0.39 & 0.48 & 0.39 & 2,807 & 1,413 & 81 & 1 \\ \hline
    \hline
    24,868 & 2.6 & 37.9 & 0.04 & 0.05 & 0.05 & 1.70 & 0.04 & 1 & 1 & 1 & 1 \\ \hline
  \end{tabular}

  \medskip
  %% \begin{minipage}{\textwidth}
  %%   Instances are grouped by intended average degree: 4, 8, 16, 32, and 64,
  %%   respectively, undershot for the larger degrees.
  %%   The configurations shown include, for each instance, at least one of the
  %%   minimum runtimes.
  %%   For the sparsest graphs, \domRed{} is effective because there are many
  %%   dominated degree-3 vertices -- see Fig.~\ref{fig:geo_drawings}.
  %%   At higher densities, \unconfinedRed{} reductions are useful. In the mid-range
  %%   -- average degree roughly 32, normalized to 11 -- CPLEX is the better
  %%   choice; unconfined reductions (and our other configurations)
  %%   are less effective. At the highest density, there are enough large
  %%   cliques so that \domRed{} can reduce the graph at the root.
    
  %%   All of these instances are easy for CPLEX -- the only reason it does not
  %%   always have the best runtimes is because of row and column elimination at
  %%   the root.
  %% \end{minipage}
\end{table*}

% [Last modified: 2019 08 15 at 16:35:14 GMT]


==> Y-none-table.tex <==
\begin{table}
  \caption{Selected instances in the \none{} region.}
  \label{tab:none-table}
  \begin{tabular}{|r|r||r|r|r|r|r|r|r|r|}
    \hline
spread & nad & None & Deg1 & DD & Cheap & LP & All & CPLEX & min\\\hline
0.68 & 160 & \textbf{0.83} & \textbf{0.76} & 2.16 & 2.24 & \textbf{0.95} & 2.31 & 13.33 & 0.76\\\hline
0.04 & 80 & \textbf{4.90} & \textbf{6.52} & \textbf{6.80} & \emph{7.74} & 9.24 & 18.22 & 243.38 & 4.91\\\hline
0.19 & 80 & \textbf{3.68} & \textbf{4.24} & \textbf{4.83} & \emph{5.78} & 6.28 & 13.06 & 103.86 & 3.69\\\hline
1.5 & 80 & \textbf{1.89} & \textbf{2.52} & \textbf{1.97} & 3.07 & 3.15 & 5.26 & 137.06 & 1.89\\\hline
2.13 & 80 & \textbf{2.49} & \textbf{1.93} & \textbf{2.29} & 3.19 & 3.28 & 5.68 & 151.98 & 1.93\\\hline
1.53 & 80 & \textbf{6.16} & \textbf{5.72} & 8.14 & 9.1 & 10.14 & 21.53 & 859.97 & 5.73\\\hline
\end{tabular}
\end{table}

% [Last modified: 2019 02 28 at 19:35:42 GMT]


==> Y-none_is_best.tex <==
\begin{table*}
  \caption{Selected instances where the best runtimes are achieved with no reductions.}
  \label{tab:none-table}

  \medskip
  \begin{center}
  \begin{tabular}{|l||r|r|r|r|r|r|}
    \hline
    Instance & None & r0\_l1 & r1\_l4 & r2\_l4 & r3\_l4 & CPLEX \\ \hline
%    gka\_28 & 84.45 & 114.04 & 256.95 & 403.02 & 455.83 & 611.78  \\ \hline
    san1000 & 30.93 & 87.99 & 176.32 & 305.46 & 762.71 & t/o  \\ \hline
    DSJC1000.9 & 27.90 & 91.33 & 111.42 & 232.12 & 699.34 & t/o  \\ \hline
    p\_hat700-1 & 12.47 & 32.99 & 58.04 & 97.47 & 218.92 & t/o \\ \hline
    c-fat500-1 & 2.26 & 4.57 & 4.80 & 7.29 & 7.32 & 71.92  \\ \hline
%    gka\_33 & 1.58 & 3.88 & 5.48 & 7.80 & 9.38 & 12.58  \\ \hline
  \end{tabular}

  \medskip
  \begin{tabular}{|l||r|r|r|r|r|r|r|r|r|r|r|}
    \hline
    Instance & n & m & min & bot & med & mean & top & max & stdev & nad & t/b \\ \hline
    gka\_28 & 200 & 2,950 & 18 & 23 & 29 & 29.5 & 38 & 41 & 4.6 & 29.5 & 1.66 \\ \hline
    san1000 & 1,0 & 249,0 & 449 & 462 & 484 & 498.0 & 536 & 554 & 28.3 & 99.6 & 1.16 \\ \hline
    DSJC1000.9 & 1,0 & 449,449 & 870 & 883 & 899 & 898.9 & 914 & 924 & 9.6 & 179.8 & 1.04 \\ \hline
    p\_hat700-1 & 700 & 183,651 & 413 & 440 & 525 & 524.7 & 606 & 624 & 53.0 & 149.9 & 1.38 \\ \hline
    c-fat500-1 & 500 & 120,291 & 479 & 479 & 482 & 481.2 & 482 & 482 & 1.3 & 192.5 & 1.01 \\ \hline
    gka\_33 & 200 & 7,914 & 68 & 72 & 79 & 79.1 & 87 & 88 & 4.6 & 79.1 & 1.21 \\ \hline
  \end{tabular}
  \end{center}

  \medskip
  \begin{minipage}{\textwidth}
    The top table shows that doing no reductions yields the best runtimes for
    some instances (these are not the only ones), and increasing number of
    reductions makes matters worse. CPLEX also does really badly on these
    instances.

    The bottom table shows that, except for the first instance, all of these
    are dense and have very little degree variation \cmt{where to introduce
      'spread' for top/bottom?}. The first instance differs in that runtime
    for r0\_l1 is within $1.5$ of None. 
  \end{minipage}
\end{table*}

% [Last modified: 2019 07 24 at 14:30:54 GMT]


==> Y-none_region.tex <==
\begin{table}
  \caption{Runtime data for instances where it pays to do no reductions at all.}
  \label{tab:none_region}

  \medskip
  \begin{tabular}{|l||r|r|r|r||r|r|r|r|r|}
    \hline
    Instance & n & m & spread & nad & \none{} & \dft{} & \rOlI{} & min & CPLEX \\ \hline
p\_hat1500-1 & 1,500 & 839,327 & 1.36 & 149.21 & 430.79 & 465.10 & 900.01 & 430.79 & t/o \\ \hline
DSJC500.5 & 500 & 62,624 & 1.15 & 100.20 & 115.74 & 127.01 & 205.24 & 115.74 & t/o \\ \hline
san400\_0.7\_2 & 400 & 23,940 & 1.23 & 59.85 & 50.93 & 56.28 & 89.06 & 50.93 & 727.01 \\ \hline
p\_hat1000-1 & 1,000 & 377,247 & 1.35 & 150.90 & 48.49 & 52.19 & 135.30 & 48.49 & t/o \\ \hline
san1000 & 1,000 & 249,000 & 1.16 & 99.60 & 30.93 & 34.50 & 87.99 & 30.93 & t/o \\ \hline
p\_hat700-1 & 700 & 183,651 & 1.38 & 149.92 & 12.47 & 12.90 & 32.99 & 12.47 & t/o \\ \hline
p\_hat500-2 & 500 & 61,804 & 2.62 & 98.89 & 10.53 & 11.42 & 19.11 & 10.53 & t/o \\ \hline
p\_hat500-1 & 500 & 93,181 & 1.37 & 149.09 & 5.12 & 5.65 & 10.75 & 5.12 & t/o \\ \hline
DSJC500.9 & 500 & 112,437 & 1.05 & 179.90 & 3.60 & 4.15 & 9.10 & 3.60 & t/o \\ \hline
gka\_30-to-7 & 200 & 4,964 & 1.40 & 49.28 & 3.23 & 3.93 & 5.81 & 3.23 & 13.55 \\ \hline
ba\_256\_084\_3 & 256 & 8,988 & 3.17 & 54.86 & 2.03 & 3.46 & 3.53 & 2.03 & 31.38 \\ \hline
gka\_32 & 200 & 6,968 & 1.31 & 68.34 & 1.96 & 3.37 & 4.02 & 1.96 & 46.43 \\ \hline
  \end{tabular}

  \medskip
  \begin{minipage}{\textwidth}
    These are sorted by decreasing runtime for \none{}.
    The main contrast here is between \none{} and \rOlI{}, even more so with
    CPLEX.
    The \dft{} configuration does almost as well as \none{} -- the two
    reductions involved take little time and may reduce the number of branches.
    Note, too, that \rOlI{} is competitive on instances with smaller nad.
    
    \cmt{add a comment about branches?}
  \end{minipage}
\end{table}

% [Last modified: 2019 07 25 at 20:24:34 GMT]


==> Y-none_vs_all.tex <==
\begin{table*}
\small
  
  \caption{Instances that show a sharp contrast between runtimes for doing no
    reductions versus doing all reductions.}
  \label{tab:none_vs_all}

  \medskip
  \begin{center}

    \input{Y-none_table}

    \medskip
    (a) Instances with better runtimes when no reductions are done.
    
    \medskip
    \input{Y-all_table}

    \medskip
    (b) Instances with better runtimes when all reductions are done.

  \end{center}
  
  Runs with None use no reductions and a clique cover lower
  bound only; runs with All use all reductions except \packingRed{} and all lower
  bounds except cycle cover.
  Time out (t-o) is 900~seconds. Sources of the
  instances are described in Section~\ref{sec:instances}.
  
\end{table*}

% [Last modified: 2020 02 18 at 15:27:27 GMT]


==> Y-packing.tex <==
\begin{table}
  \caption{Packing complicates branching.}
  \label{tab:packing}

  \centering
  \small
  \medskip
  \begin{tabular}{|l||r|r|r|r||r|}
    \hline
    \multicolumn{6}{|c|}{runtime} \\
    \hline
    Instance & None & r0\_l1 & r1\_l4 & r2\_l4 & r3\_l4 \\ \hline
aa42-to & 242.74 & 89.82 & 7.19 & 10.30 & $> 7200$ \\ \hline
san400\_0.7\_1 & 19.83 & 32.47 & 89.91 & 122.46 & 2626.54 \\ \hline
ba\_256\_090 & 0.97 & 1.91 & 3.48 & 4.56 & 26.97 \\ \hline\hline
\multicolumn{6}{|c|}{branches} \\ \hline
Instance & None & r0\_l1 & r1\_l4 & r2\_l4 & r3\_l4 \\ \hline
aa42-to & 3,982,877 & 496,173 & 12,428 & 12,089 & $> 9,338,420$ \\ \hline
san400\_0.7\_1 & 144,025 & 141,591 & 141,289 & 140,489 & 2,208,544 \\ \hline
ba\_256\_090 & 3,240 & 2,597 & 2,554 & 2,520 & 64,548 \\ \hline
  \end{tabular}

  \medskip
  \begin{minipage}{\textwidth}
    Early on, we took packing reductions out of the mix. Packing injects a
    different branching strategy that, in many cases, can wreak
    havoc. Table~\ref{tab:packing} shows three
    of the most egregious examples. The r3\_l4 configuration differs from
    r2\_l4 only in that the former includes packing.
  \end{minipage}

\end{table}

% [Last modified: 2019 07 22 at 16:58:01 GMT]


==> Y-platform_runtimes.tex <==
\begin{table*}
  \caption{Runtime variations among different platforms.}
  \label{tab:platform_runtimes}

  \medskip
  \begin{minipage}{\textwidth}
    \tiny
    \begin{center}
      \begin{tabular}{|l||r|r|r|r||r|r|r|r||r|r|r||r|}
        \hline
        & \multicolumn{4}{c||}{All}
        & \multicolumn{4}{c||}{None}
        & \multicolumn{3}{c||}{All/None}
        & 
        \\
        \cline{1-12}
        instance
        & $cpu_1$ & $cpu_2$ & $cpu_3$ & branches
        & $cpu_1$ & $cpu_2$ & $cpu_3$ & branches
        & $cpu_1$ & $cpu_2$ & $cpu_3$ 
        & \emph{max}
        \\
        \hline\hline
        blg-200\_40\_00
        & 661.11
        & 499.43
        & 503.00
        & 4,521,973 & 156.00 & 118.78 & 116.04 & 5,282,886 & 4.238 &
        \textbf{\emph{4.205}} & \textbf{4.335} & 1.03\\\hline
        san1000 & 214.33 & 153.27 & 139.42 & 125,380 & 32.84 & 22.65 & 21.42
        & 229,242 & 6.527 & \textbf{\emph{6.767}} & \textbf{\emph{6.509}} &
        1.04\\\hline
        p\_hat1000-1 & 316.05 & 228.57 & 208.05 & 409,285 & 47.95 & 36.05 &
        35.59 & 421,894 & \textbf{6.591} & 6.341 &
        \textbf{\emph{5.846}} & 1.13\\\hline 
        gka\_32 & 6.22 & 4.13 & 4.78 & 11,536 & 2.17 & 1.28 & 1.56 & 22,010 &
        \textbf{\emph{2.863}} & \textbf{3.232} & 3.057 & 1.13\\\hline
        aa20-cl & 1.48 & 0.91 & 1.48 & 2,201 & 5.08 & 3.49 & 4.78 & 494,612 &
        0.291 & \textbf{\emph{0.261}} & \textbf{0.309} & 1.19\\\hline 
        blg-200\_10\_01 & 16.49 & 9.81 & 13.02 & 82,757 & 303.12 & 208.85 &
        213.25 & 23,313,504 & 0.054 & \textbf{\emph{0.047}} &
        \textbf{0.061} & 1.30\\\hline 
      \end{tabular}
    \end{center}
  \end{minipage}

  \medskip
    \begin{minipage}{\textwidth}
      Each ratio column shows the ratio between the None and All runtimes.
      The \emph{max}
      column shows the maximum ratio among the All/None ratios, i.e., the max of
      $cpu_1 / cpu_2$, $cpu_1 / cpu_3$, and $cpu_2 / cpu_3$, and their
      inverses. The larger of two ratios achieving the max are is in bold
      font, the smaller in bold italic.
    \end{minipage}

    \bigskip
    \begin{minipage}{\textwidth}
      \begin{center}
      \begin{tabular}{|r|c|c|r|r|r|}
        \hline
        id & \multicolumn{1}{c|}{processor -- all Intel(R)}
        & \multicolumn{1}{c|}{processor -- all Linux/Unix} & speed & cache & memory \\
        \hline\hline
        $cpu_1$ & Xeon(R) E5645 & Red Hat 4.8.5 & 2.40GHz & 12 MB & 4 GB \\
        \hline
        $cpu_2$ & Xeon(R) E5-2695 v2 & Ubuntu 4.15.0 & 2.40GHz & 30 MB & 128 GB \\
        \hline
        $cpu_3$ & Core i7 & macOS 10.12.6 & 2.20GHz & 4 MB\footnote{L3 cache, 256
          KB L2 cache} & 8 GB \\
        \hline
      \end{tabular}
      \end{center}
    \end{minipage}

    \bigskip
    \begin{minipage}{\textwidth}
      \begin{center}
        \begin{tabular}{|l|r|r|r|r|r|r|r|}
          \hline
          & \multicolumn{7}{c|}{degree statistics} \\
          \cline{2-8}
          instance & $n$ & $m$ & min & median & mean & max & stdev \\
          \hline\hline
          aa20-cl & 450 & 1721 & 1 & 3 & 7.6 & 38 & 9.2\\\hline
          blg-200\_10\_01 & 200 & 1000 & 5 & 7 & 10.0 & 20 & 6.2\\\hline
          blg-200\_40\_00 & 200 & 4000 & 39 & 40 & 40.0 & 41 & 0.1\\\hline
          gka\_32 & 200 & 6968 & 57 & 70 & 69.7 & 82 & 4.5\\\hline
          p\_hat1000-1 & 1000 & 377247 & 591 & 754 & 754.5 & 894 & 73.3\\\hline
          san1000 & 1000 & 249000 & 449 & 484 & 498.0 & 554 & 28.3\\\hline
        \end{tabular}
      \end{center}
    \end{minipage}

    \bigskip
    \begin{minipage}{\textwidth}
      Observations:
      \begin{itemize}
      \item
        The statistics, along with those in
        Table~\ref{tab:permutation_runtimes} justify a $1.25$ competitive
        ratio instead of the $1.5$ currently in use.
      \item
        Runtimes for $cpu_3$ are often fastest because the processor is
        adaptive -- runs faster than advertised speed under ideal conditions.
      \item
        Cache size matters. The ratio for $cpu_3$ is largest, and the
        difference in ratio between $cpu_2$ and $cpu_3$ greatest, when the
        difference in number of branches is greatest. See the last two lines
        of the table.
      \end{itemize}
    \end{minipage}
\end{table*}

\begin{table*}
  \caption{Runtime variations when inputs are permuted.}
  \label{tab:permutation_runtimes}

  \medskip
  \begin{minipage}{\textwidth}
  \begin{center}
      \begin{tabular}{|l||r|r|r|r|r|c|c|}
        \hline
        instance & min & med & mean & max & stdev
        & $+/-$ \footnote{ratio between one stdev greater than mean and one
          stdev less than mean}
        & max/min
        \\
        \hline\hline
        \texttt{aa41-cl} & 13.01 & 14.64 & 14.76 & 16.14 & 0.75 & 1.10 & 1.24
        \\
        \hline
        \texttt{reg3-300} & 11.11 & 14.84 & 14.41 & 17.08 & 1.47 & 1.22 & 1.54
        \\
        \hline
      \end{tabular}
  \end{center}
  \end{minipage}
\end{table*}

% [Last modified: 2019 06 28 at 14:44:26 GMT]


==> Y-reduction-effectiveness.tex <==
\begin{figure}
  \centering

  % the chart is in file reductions-blg-none.xlsx in 0-blg_processing; it's
  % not clear, however, where the numbers come from
  \includegraphics[width=0.8\textwidth]{reduction-effectiveness}
  
  \caption{Effectiveness of various reductions on instances in each region.}
  \label{fig:reduction-effectiveness}
\end{figure}

% [Last modified: 2020 02 18 at 15:27:26 GMT]


==> Y-reductions.tex <==
\begin{table}%[ht]
    \caption{Time complexity and original author for various reductions.}
    \label{tab:reductions}

    \cmt{(References are comments in source) possibly include packing}

    \centering
    \begin{tabular}{|l|@{\hskip 0.5in}r|}
        \hline
        \bf Reduction & \bf Complexity\\
        \hline
        \degRed{} & $O(n)$\\
        \domRed{} & $O(n^3)$\\
        \unconfinedRed{} & $O(n^4)$\\ % Xiao13/17 
        \lpRed{} (Initial) & $O(m\sqrt{n})$\\ %HopkroftKarp/maxflow
        \lpRed{} (Update) & $O(m + n)$\\ %Iwata14
        \foldRed{} & $O(m)$\\ %Xiao13/17 and Fomin09
        \twinRed{} & $O(m)$\\ %Xiao13/17
        \deskRed{} & $O(m)$\\ %Xiao13/17
        \funnelRed{} & $O(mn)$\\ %Xiao13/17
        \hline
    \end{tabular}
\end{table}

% [Last modified: 2018 08 09 at 19:16:35 GMT]


==> Y-tensor.tex <==
\begin{table}
  \caption{Runtimes for tensor networks}
  \label{tab:tensor}

  \medskip
  \begin{minipage}{\textwidth}
    \begin{tabular}{|r|r|r|r|r|}
      \hline
      \multicolumn{1}{|c|}{instance~\footnote{In the name $a \times b$\_$c$,
          the $a$ and $b$ refer to the
          dimensions of the network and the $c$ to its number of \emph{fermions}.}}
      & 
      \multicolumn{1}{c|}{\dd}
      &
      \multicolumn{1}{c|}{Ch+U\footnote{Cheap reductions plus unconfined.}}
      &
      \multicolumn{1}{c|}{\all}
      &
      \multicolumn{1}{c|}{CPLEX}
      \\
      \hline
      $4\times 4\_33$ & 13.1 & 2.3 & 2.4 & 0.04 
      \\
      \hline
      $4\times 4\_34$ & 3.8 & 0.5 & 0.4 & 0.05
      \\
      \hline
      $4\times 4\_35$ & 4.8 & 1.0 & 1.0 & 0.02
      \\
      \hline
      $4\times 4\_36$ & 6.2 & 1.5 & 1.0 & 0.03
      \\
      \hline
      $4\times 5\_26$  & $\approx 0.01$ & $\approx 0.01$ & $\approx 0.01$ & 0.02 
      \\
      \hline
    \end{tabular}

  \medskip
  Each entry is a median of ten trials on different (random) networks. All of
  these
  networks have 401 to 448 vertices,
  average degree ranging from 3.6 to 3.8 and degree spread from
  2.92 to 2.96.
  \end{minipage}
\end{table}

% [Last modified: 2019 02 15 at 17:19:35 GMT]


==> Y-unconfined.tex <==
\begin{figure}
  A vertex is \emph{unconfined} if the following algorithm returns true.
\begin{enumerate}
\item $S = {v}$.
\item Find $u \in N(S)$ with $|N(u) \cap S| = 1$ and having minimum value of $|N(u) \setminus N[S]|$.
\item If no such $u$ exists or $|N(u) \setminus N[S]| > 1$, return false. \label{stepo:confined}
\item If $N(u) \setminus N[S] = \emptyset$, return true. \label{step:unconfined}
\item Otherwise, $S = S \cup (N(u) \setminus N[S])$ and start again from step 2.
\end{enumerate}

\caption{Algorithm for identifying an unconfined vertex.}
\label{fig:unconfined}
\end{figure}

% [Last modified: 2019 02 28 at 17:22:40 GMT]

